Trapped Bose gases with large positive scattering length

We calculate the energy and the condensate fraction of a system of trapped bosons interacting via a short-range two-body potential with positive scattering length. The potential is attractive and has a two-body bound state. When the scattering length is small compared to the trap length the system is model independent: all potential models -- attractive, repulsive and zero-range -- provide similar results. When the scattering length is large the attractive model differs qualitatively from the repulsive and zero-range models. In this regime the system with attractive potential becomes independent of the scattering length, with both the energy and the condensate fraction converging towards finite constants.

==> fig-cd.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup%
  \makeatletter%
  \newcommand{\GNUPLOTspecial}{%
    \@sanitize\catcode`\%=14\relax\special}%
  \setlength{\unitlength}{0.1bp}%
{\GNUPLOTspecial{!
%!PS-Adobe-2.0
%%Title: ../fig-cd.tex
%%Creator: gnuplot 3.7 patchlevel 3
%%CreationDate: Tue May 22 12:32:14 2007
%%DocumentFonts: 
%%BoundingBox: 0 0 216 162
%%Orientation: Landscape
%%Pages: (atend)
%%EndComments
/gnudict 256 dict def
gnudict begin
/Color false def
/Solid false def
/gnulinewidth 5.000 def
/userlinewidth gnulinewidth def
/vshift -33 def
/dl {10 mul} def
/hpt_ 31.5 def
/vpt_ 31.5 def
/hpt hpt_ def
/vpt vpt_ def
/M {moveto} bind def
/L {lineto} bind def
/R {rmoveto} bind def
/V {rlineto} bind def
/vpt2 vpt 2 mul def
/hpt2 hpt 2 mul def
/Lshow { currentpoint stroke M
  0 vshift R show } def
/Rshow { currentpoint stroke M
  dup stringwidth pop neg vshift R show } def
/Cshow { currentpoint stroke M
  dup stringwidth pop -2 div vshift R show } def
/UP { dup vpt_ mul /vpt exch def hpt_ mul /hpt exch def
  /hpt2 hpt 2 mul def /vpt2 vpt 2 mul def } def
/DL { Color {setrgbcolor Solid {pop []} if 0 setdash }
 {pop pop pop Solid {pop []} if 0 setdash} ifelse } def
/BL { stroke userlinewidth 2 mul setlinewidth } def
/AL { stroke userlinewidth 2 div setlinewidth } def
/UL { dup gnulinewidth mul /userlinewidth exch def
      dup 1 lt {pop 1} if 10 mul /udl exch def } def
/PL { stroke userlinewidth setlinewidth } def
/LTb { BL [] 0 0 0 DL } def
/LTa { AL [1 udl mul 2 udl mul] 0 setdash 0 0 0 setrgbcolor } def
/LT0 { PL [] 1 0 0 DL } def
/LT1 { PL [4 dl 2 dl] 0 1 0 DL } def
/LT2 { PL [2 dl 3 dl] 0 0 1 DL } def
/LT3 { PL [1 dl 1.5 dl] 1 0 1 DL } def
/LT4 { PL [5 dl 2 dl 1 dl 2 dl] 0 1 1 DL } def
/LT5 { PL [4 dl 3 dl 1 dl 3 dl] 1 1 0 DL } def
/LT6 { PL [2 dl 2 dl 2 dl 4 dl] 0 0 0 DL } def
/LT7 { PL [2 dl 2 dl 2 dl 2 dl 2 dl 4 dl] 1 0.3 0 DL } def
/LT8 { PL [2 dl 2 dl 2 dl 2 dl 2 dl 2 dl 2 dl 4 dl] 0.5 0.5 0.5 DL } def
/Pnt { stroke [] 0 setdash
   gsave 1 setlinecap M 0 0 V stroke grestore } def
/Dia { stroke [] 0 setdash 2 copy vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath stroke
  Pnt } def
/Pls { stroke [] 0 setdash vpt sub M 0 vpt2 V
  currentpoint stroke M
  hpt neg vpt neg R hpt2 0 V stroke
  } def
/Box { stroke [] 0 setdash 2 copy exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V closepath stroke
  Pnt } def
/Crs { stroke [] 0 setdash exch hpt sub exch vpt add M
  hpt2 vpt2 neg V currentpoint stroke M
  hpt2 neg 0 R hpt2 vpt2 V stroke } def
/TriU { stroke [] 0 setdash 2 copy vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath stroke
  Pnt  } def
/Star { 2 copy Pls Crs } def
/BoxF { stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V  hpt2 0 V  0 vpt2 V
  hpt2 neg 0 V  closepath fill } def
/TriUF { stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath fill } def
/TriD { stroke [] 0 setdash 2 copy vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath stroke
  Pnt  } def
/TriDF { stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath fill} def
/DiaF { stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath fill } def
/Pent { stroke [] 0 setdash 2 copy gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath stroke grestore Pnt } def
/PentF { stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath fill grestore } def
/Circle { stroke [] 0 setdash 2 copy
  hpt 0 360 arc stroke Pnt } def
/CircleF { stroke [] 0 setdash hpt 0 360 arc fill } def
/C0 { BL [] 0 setdash 2 copy moveto vpt 90 450  arc } bind def
/C1 { BL [] 0 setdash 2 copy        moveto
       2 copy  vpt 0 90 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C2 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 90 180 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C3 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 0 180 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C4 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 180 270 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C5 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 0 90 arc
       2 copy moveto
       2 copy  vpt 180 270 arc closepath fill
               vpt 0 360 arc } bind def
/C6 { BL [] 0 setdash 2 copy moveto
      2 copy  vpt 90 270 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C7 { BL [] 0 setdash 2 copy moveto
      2 copy  vpt 0 270 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C8 { BL [] 0 setdash 2 copy moveto
      2 copy vpt 270 360 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C9 { BL [] 0 setdash 2 copy moveto
      2 copy  vpt 270 450 arc closepath fill
              vpt 0 360 arc closepath } bind def
/C10 { BL [] 0 setdash 2 copy 2 copy moveto vpt 270 360 arc closepath fill
       2 copy moveto
       2 copy vpt 90 180 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C11 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 0 180 arc closepath fill
       2 copy moveto
       2 copy  vpt 270 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C12 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 180 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C13 { BL [] 0 setdash  2 copy moveto
       2 copy  vpt 0 90 arc closepath fill
       2 copy moveto
       2 copy  vpt 180 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/C14 { BL [] 0 setdash 2 copy moveto
       2 copy  vpt 90 360 arc closepath fill
               vpt 0 360 arc } bind def
/C15 { BL [] 0 setdash 2 copy vpt 0 360 arc closepath fill
               vpt 0 360 arc closepath } bind def
/Rec   { newpath 4 2 roll moveto 1 index 0 rlineto 0 exch rlineto
       neg 0 rlineto closepath } bind def
/Square { dup Rec } bind def
/Bsquare { vpt sub exch vpt sub exch vpt2 Square } bind def
/S0 { BL [] 0 setdash 2 copy moveto 0 vpt rlineto BL Bsquare } bind def
/S1 { BL [] 0 setdash 2 copy vpt Square fill Bsquare } bind def
/S2 { BL [] 0 setdash 2 copy exch vpt sub exch vpt Square fill Bsquare } bind def
/S3 { BL [] 0 setdash 2 copy exch vpt sub exch vpt2 vpt Rec fill Bsquare } bind def
/S4 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt Square fill Bsquare } bind def
/S5 { BL [] 0 setdash 2 copy 2 copy vpt Square fill
       exch vpt sub exch vpt sub vpt Square fill Bsquare } bind def
/S6 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt vpt2 Rec fill Bsquare } bind def
/S7 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt vpt2 Rec fill
       2 copy vpt Square fill
       Bsquare } bind def
/S8 { BL [] 0 setdash 2 copy vpt sub vpt Square fill Bsquare } bind def
/S9 { BL [] 0 setdash 2 copy vpt sub vpt vpt2 Rec fill Bsquare } bind def
/S10 { BL [] 0 setdash 2 copy vpt sub vpt Square fill 2 copy exch vpt sub exch vpt Square fill
       Bsquare } bind def
/S11 { BL [] 0 setdash 2 copy vpt sub vpt Square fill 2 copy exch vpt sub exch vpt2 vpt Rec fill
       Bsquare } bind def
/S12 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill Bsquare } bind def
/S13 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill
       2 copy vpt Square fill Bsquare } bind def
/S14 { BL [] 0 setdash 2 copy exch vpt sub exch vpt sub vpt2 vpt Rec fill
       2 copy exch vpt sub exch vpt Square fill Bsquare } bind def
/S15 { BL [] 0 setdash 2 copy Bsquare fill Bsquare } bind def
/D0 { gsave translate 45 rotate 0 0 S0 stroke grestore } bind def
/D1 { gsave translate 45 rotate 0 0 S1 stroke grestore } bind def
/D2 { gsave translate 45 rotate 0 0 S2 stroke grestore } bind def
/D3 { gsave translate 45 rotate 0 0 S3 stroke grestore } bind def
/D4 { gsave translate 45 rotate 0 0 S4 stroke grestore } bind def
/D5 { gsave translate 45 rotate 0 0 S5 stroke grestore } bind def
/D6 { gsave translate 45 rotate 0 0 S6 stroke grestore } bind def
/D7 { gsave translate 45 rotate 0 0 S7 stroke grestore } bind def
/D8 { gsave translate 45 rotate 0 0 S8 stroke grestore } bind def
/D9 { gsave translate 45 rotate 0 0 S9 stroke grestore } bind def
/D10 { gsave translate 45 rotate 0 0 S10 stroke grestore } bind def
/D11 { gsave translate 45 rotate 0 0 S11 stroke grestore } bind def
/D12 { gsave translate 45 rotate 0 0 S12 stroke grestore } bind def
/D13 { gsave translate 45 rotate 0 0 S13 stroke grestore } bind def
/D14 { gsave translate 45 rotate 0 0 S14 stroke grestore } bind def
/D15 { gsave translate 45 rotate 0 0 S15 stroke grestore } bind def
/DiaE { stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V closepath stroke } def
/BoxE { stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V closepath stroke } def
/TriUE { stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V closepath stroke } def
/TriDE { stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V closepath stroke } def
/PentE { stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  closepath stroke grestore } def
/CircE { stroke [] 0 setdash 
  hpt 0 360 arc stroke } def
/Opaque { gsave closepath 1 setgray fill grestore 0 setgray closepath } def
/DiaW { stroke [] 0 setdash vpt add M
  hpt neg vpt neg V hpt vpt neg V
  hpt vpt V hpt neg vpt V Opaque stroke } def
/BoxW { stroke [] 0 setdash exch hpt sub exch vpt add M
  0 vpt2 neg V hpt2 0 V 0 vpt2 V
  hpt2 neg 0 V Opaque stroke } def
/TriUW { stroke [] 0 setdash vpt 1.12 mul add M
  hpt neg vpt -1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt 1.62 mul V Opaque stroke } def
/TriDW { stroke [] 0 setdash vpt 1.12 mul sub M
  hpt neg vpt 1.62 mul V
  hpt 2 mul 0 V
  hpt neg vpt -1.62 mul V Opaque stroke } def
/PentW { stroke [] 0 setdash gsave
  translate 0 hpt M 4 {72 rotate 0 hpt L} repeat
  Opaque stroke grestore } def
/CircW { stroke [] 0 setdash 
  hpt 0 360 arc Opaque stroke } def
/BoxFill { gsave Rec 1 setgray fill grestore } def
/Symbol-Oblique /Symbol findfont [1 0 .167 1 0 0] makefont
dup length dict begin {1 index /FID eq {pop pop} {def} ifelse} forall
currentdict end definefont pop
end
%%EndProlog
}}%
\begin{picture}(2160,1620)(0,0)%
{\GNUPLOTspecial{"
%%Page: 1 1
gnudict begin
gsave
0 0 translate
0.100 0.100 scale
0 setgray
newpath
1.000 UL
LTb
450 300 M
63 0 V
1497 0 R
-63 0 V
450 522 M
63 0 V
1497 0 R
-63 0 V
450 744 M
63 0 V
1497 0 R
-63 0 V
450 965 M
63 0 V
1497 0 R
-63 0 V
450 1187 M
63 0 V
1497 0 R
-63 0 V
450 1409 M
63 0 V
1497 0 R
-63 0 V
450 300 M
0 31 V
0 1189 R
0 -31 V
536 300 M
0 31 V
0 1189 R
0 -31 V
598 300 M
0 31 V
0 1189 R
0 -31 V
645 300 M
0 31 V
0 1189 R
0 -31 V
684 300 M
0 31 V
0 1189 R
0 -31 V
717 300 M
0 31 V
0 1189 R
0 -31 V
746 300 M
0 31 V
0 1189 R
0 -31 V
771 300 M
0 31 V
0 1189 R
0 -31 V
793 300 M
0 63 V
0 1157 R
0 -63 V
941 300 M
0 31 V
0 1189 R
0 -31 V
1028 300 M
0 31 V
0 1189 R
0 -31 V
1089 300 M
0 31 V
0 1189 R
0 -31 V
1137 300 M
0 31 V
0 1189 R
0 -31 V
1176 300 M
0 31 V
0 1189 R
0 -31 V
1208 300 M
0 31 V
0 1189 R
0 -31 V
1237 300 M
0 31 V
0 1189 R
0 -31 V
1262 300 M
0 31 V
0 1189 R
0 -31 V
1284 300 M
0 63 V
0 1157 R
0 -63 V
1432 300 M
0 31 V
0 1189 R
0 -31 V
1519 300 M
0 31 V
0 1189 R
0 -31 V
1580 300 M
0 31 V
0 1189 R
0 -31 V
1628 300 M
0 31 V
0 1189 R
0 -31 V
1667 300 M
0 31 V
0 1189 R
0 -31 V
1700 300 M
0 31 V
0 1189 R
0 -31 V
1728 300 M
0 31 V
0 1189 R
0 -31 V
1753 300 M
0 31 V
0 1189 R
0 -31 V
1776 300 M
0 63 V
0 1157 R
0 -63 V
1924 300 M
0 31 V
0 1189 R
0 -31 V
2010 300 M
0 31 V
0 1189 R
0 -31 V
1.000 UL
LTb
450 300 M
1560 0 V
0 1220 V
-1560 0 V
450 300 L
0.500 UP
1.000 UL
LT3
1955 674 Box
1889 542 Box
1839 446 Box
1798 399 Box
1764 402 Box
1686 533 Box
1665 581 Box
1646 626 Box
1517 913 Box
1437 1047 Box
1380 1123 Box
1336 1172 Box
1243 1254 Box
768 1391 Box
1056 633 Box
0.500 UP
1.000 UL
LT4
1806 1046 BoxF
1676 708 BoxF
1597 642 BoxF
1540 789 BoxF
1496 900 BoxF
1281 1216 BoxF
1056 533 BoxF
0.500 UP
1.000 UL
LT5
1766 1234 Circle
1687 1146 Circle
1630 1054 Circle
1586 904 Circle
1493 811 Circle
1449 932 Circle
1371 1092 Circle
1317 1166 Circle
1056 433 Circle
1.000 UL
LT3
450 1405 M
12 0 V
15 -1 V
16 0 V
15 0 V
15 -1 V
15 0 V
16 0 V
15 -1 V
15 0 V
15 -1 V
16 -1 V
15 0 V
15 -1 V
15 -1 V
16 0 V
15 -1 V
15 -1 V
15 -1 V
15 -1 V
16 -1 V
15 -1 V
15 -2 V
15 -1 V
16 -1 V
15 -2 V
15 -2 V
15 -2 V
16 -2 V
15 -2 V
15 -2 V
15 -2 V
16 -3 V
15 -3 V
15 -2 V
15 -4 V
16 -3 V
15 -4 V
15 -3 V
15 -5 V
15 -4 V
16 -5 V
15 -5 V
15 -5 V
15 -6 V
16 -6 V
15 -7 V
15 -7 V
15 -8 V
16 -8 V
15 -9 V
15 -10 V
15 -10 V
16 -11 V
15 -12 V
15 -13 V
15 -13 V
16 -15 V
15 -15 V
15 -16 V
15 -17 V
15 -17 V
16 -19 V
15 -19 V
15 -21 V
15 -22 V
16 -23 V
15 -25 V
15 -25 V
15 -27 V
16 -28 V
15 -29 V
15 -31 V
15 -32 V
16 -33 V
15 -34 V
15 -35 V
15 -36 V
15 -36 V
16 -37 V
15 -36 V
15 -36 V
15 -34 V
16 -32 V
15 -28 V
15 -24 V
15 -18 V
16 -10 V
15 -2 V
15 6 V
15 15 V
16 20 V
15 26 V
15 28 V
15 31 V
16 31 V
15 31 V
15 29 V
15 30 V
15 31 V
1.000 UL
LT4
1281 1216 M
5 -5 V
5 -4 V
6 -5 V
5 -5 V
5 -6 V
6 -5 V
5 -5 V
5 -6 V
5 -5 V
6 -6 V
5 -6 V
5 -6 V
6 -6 V
5 -7 V
5 -6 V
6 -7 V
5 -7 V
5 -7 V
5 -7 V
6 -8 V
5 -7 V
5 -8 V
6 -8 V
5 -8 V
5 -9 V
6 -8 V
5 -9 V
5 -9 V
6 -9 V
5 -10 V
5 -9 V
5 -10 V
6 -10 V
5 -10 V
5 -11 V
6 -11 V
5 -11 V
5 -11 V
6 -11 V
5 -12 V
5 -12 V
5 -13 V
6 -12 V
5 -13 V
5 -13 V
6 -13 V
5 -14 V
5 -14 V
6 -15 V
5 -14 V
5 -15 V
5 -16 V
6 -15 V
5 -15 V
5 -14 V
6 -14 V
5 -14 V
5 -12 V
6 -10 V
5 -10 V
5 -7 V
6 -5 V
5 -3 V
5 -1 V
5 0 V
6 3 V
5 4 V
5 6 V
6 8 V
5 10 V
5 10 V
6 12 V
5 12 V
5 14 V
5 13 V
6 13 V
5 14 V
5 13 V
6 14 V
5 13 V
5 14 V
6 13 V
5 14 V
5 14 V
6 13 V
5 14 V
5 13 V
5 14 V
6 14 V
5 13 V
5 14 V
6 14 V
5 14 V
5 14 V
6 14 V
5 14 V
5 15 V
5 15 V
6 15 V
1.000 UL
LT5
1317 1166 M
4 -6 V
5 -5 V
5 -6 V
4 -6 V
5 -6 V
4 -6 V
5 -6 V
4 -7 V
5 -6 V
4 -7 V
5 -7 V
4 -7 V
5 -7 V
4 -8 V
5 -8 V
5 -7 V
4 -8 V
5 -9 V
4 -8 V
5 -9 V
4 -9 V
5 -10 V
4 -9 V
5 -10 V
4 -11 V
5 -10 V
4 -11 V
5 -12 V
5 -12 V
4 -12 V
5 -13 V
4 -13 V
5 -14 V
4 -13 V
5 -13 V
4 -13 V
5 -12 V
4 -11 V
5 -10 V
4 -9 V
5 -7 V
5 -6 V
4 -5 V
5 -2 V
4 -2 V
5 0 V
4 1 V
5 3 V
4 5 V
5 6 V
4 7 V
5 9 V
4 10 V
5 11 V
4 12 V
5 13 V
5 14 V
4 15 V
5 16 V
4 15 V
5 16 V
4 17 V
5 16 V
4 16 V
5 16 V
4 15 V
5 15 V
4 15 V
5 13 V
5 13 V
4 11 V
5 10 V
4 9 V
5 9 V
4 7 V
5 7 V
4 5 V
5 6 V
4 4 V
5 5 V
4 4 V
5 4 V
5 4 V
4 4 V
5 4 V
4 5 V
5 4 V
4 5 V
5 5 V
4 5 V
5 5 V
4 5 V
5 5 V
4 6 V
5 5 V
5 6 V
4 6 V
5 6 V
4 6 V
stroke
grestore
end
showpage
}}%
\put(891,433){\makebox(0,0)[r]{$N=30$}}%
\put(891,533){\makebox(0,0)[r]{$N=20$}}%
\put(891,633){\makebox(0,0)[r]{$N=10$}}%
\put(1230,50){\makebox(0,0){$(N-1)a/b_t$}}%
\put(100,910){%
\special{ps: gsave currentpoint currentpoint translate
270 rotate neg exch neg exch translate}%
\makebox(0,0)[b]{\shortstack{$n_0$, $\frac{N}{b_t^3\pi^{3/2}}$}}%
\special{ps: currentpoint grestore moveto}%
}%
\put(1776,200){\makebox(0,0){ 1}}%
\put(1284,200){\makebox(0,0){ 0.1}}%
\put(793,200){\makebox(0,0){ 0.01}}%
\put(400,1409){\makebox(0,0)[r]{ 1}}%
\put(400,1187){\makebox(0,0)[r]{ 0.9}}%
\put(400,965){\makebox(0,0)[r]{ 0.8}}%
\put(400,744){\makebox(0,0)[r]{ 0.7}}%
\put(400,522){\makebox(0,0)[r]{ 0.6}}%
\put(400,300){\makebox(0,0)[r]{ 0.5}}%
\end{picture}%
\endgroup
\endinput

